Qubits made by advanced semiconductor manufacturing

Full-scale quantum computers require the integration of millions of quantum bits. The promise of leveraging industrial semiconductor manufacturing to meet this requirement has fueled the pursuit of quantum computing in silicon quantum dots. However, to date, their fabrication has relied on electron-beam lithography and, with few exceptions, on academic style lift-off processes. Although these fabrication techniques offer process flexibility, they suffer from low yield and poor uniformity. An important question is whether the processing conditions developed in the manufacturing fab environment to enable high yield, throughput, and uniformity of transistors are suitable for quantum dot arrays and do not compromise the delicate qubit properties. Here, we demonstrate quantum dots hosted at a 28Si/28SiO2 interface, fabricated in a 300 mm semiconductor manufacturing facility using all-optical lithography and fully industrial processing. As a result, we achieve nanoscale gate patterns with remarkable homogeneity. The quantum dots are well-behaved in the multi-electron regime, with excellent tunnel barrier control, a crucial feature for fault-tolerant two-qubit gates. Single-spin qubit operation using magnetic resonance reveals relaxation times of over 1 s at 1 Tesla and coherence times of over 3 ms, matching the quality of silicon spin qubits reported to date. The feasibility of high-quality qubits made with fully-industrial techniques strongly enhances the prospects of a large-scale quantum computer

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
